Measurement of eDonkey Activity with Distributed Honeypots

Collecting information about user activity in peer-to-peer systems is a key but challenging task. We describe here a distributed platform for doing so on the eDonkey network, relying on a group of honeypot peers which claim to have certain files and log queries they receive for these files. We then conduct some measurements with typical scenarios and use the obtained data to analyze the impact of key parameters like measurement duration, number of honeypots involved, and number of advertised files. This illustrates both the possible uses of our measurement system, and the kind of data one may collect using it.

==> suite <==
\subsection{Shared files approach.}
In this section we evaluate the effectiveness of the fact that our honeypot shares lot of files,
in particular the gain obtained in terms of the number of new pairs observed per each shared files.
We consider two sets of file. First, set of popular files are those that remained popular over the 
long term duration of our trace. Second, set of random files are a subset of all files took randomly.
In addition, these files are collected from the first day 
and for both set of file, we have taken 100 files for each one.
With the same manipulation as the previous section, we calculate the number of new peers discovered, 
as a function of  shared file. We represent in what follows, the average of 100 random permutation 
and the upper and lower bound calculated from this permutation.

Figure~\ref{fig-file-pop} represent set of popular files, we observe that the file with the smallest 
value of peer is 682 and with the greatest value is 13,373. In addition, the plot of the average shows 
that we basically discover 2,700 new peer per file.\\
we also notice that the upper and lower bounds are close to the average and they have 
a similar progres. Therefore the behavior of peers in set of popular file is homogeneous.

Figure~\ref{fig-file-rand} represent set of popular files, we observe that the file with the smallest 
value of peer is 2 and with the greatest value is 11,898. In addition, the plot of the average shows 
that we basically discover 984 new peer per file.\\
we also notice that the upper and lower bounds are draw aside. 
Therefore the behavior of peers in a general case is heterogeneous 
and it depends on the type of the file searched.

\begin{figure}
  \centering
  \includegraphics[width=8.45cm]{popnb.eps}
  \caption{new peers discovered per popular file.}
  \label{fig-file-pop}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=8.45cm]{randnb.eps}
  \caption{new peers discovered per random file.}
  \label{fig-file-rand}
\end{figure}


\section{Conclusion.}
We have described a method for peer-to-peer measurement via honeypots and
implemented it on eDonkey network. This method makes it possible to collect
 rich information on peers searching for files. We have illustrated this by conducting
 some measurements  which show that we are able to attract many peers, 
and to run the measurements during long periods of time, and though avoid black listing..

 In this paper, we have evaluated two policies of our method : 
The first one consisting 
of monitoring the eDonkey network with very large honeypots, we have analysed a one month 
trace collected from 24 honeypots, and showed that, with only four shared files 
each honeypot has seen over 13 thousands peers. Morever, we have showed that the number of new peer seen 
depends on the popularity of files shared over time. 
The second policy consists of monitoring the eDonkey network with a lot of files shared, 
we have analysed a two-week trace collected by one honeypot shares files of the peers discoverd,
we also have showed that our honeypot discovers an average of 54 thousand new peers per day. 
In addition This average will be greater when more files are exposed.

 we also have evaluated two strategies for answering fike parts queries. 
we have demonstrated that the strategy random content provides the best result, 
but with disturbance of peers: it restores all parts of file download from our honeypots.

 we can conclude that monitoring the network by being attached to a large number 
of peers increases  the amount of data obtained,  and that the monitoring with different 
types of data allows to discover different communities.

 The most direct perspective of our work is To make measurements at a higher level: 
number of files, duration, distribution, and analyze the collected traces .
 In addition, we can plan to add some capabilities to our honeypots. 
For instance they can calculate popularity of their shared files during the trace.

Going further, we can plan to explore the relationships observed between peers during 
our measurement, based on the files they are trying to download. 



